Multitriangulations, pseudotriangulations and some problems of realization of polytopes

This thesis explores two specific topics of discrete geometry, the multitriangulations and the polytopal realizations of products, whose connection is the problem of finding polytopal realizations of a given combinatorial structure. A k-triangulation is a maximal set of chords of the convex n-gon such that no k+1 of them mutually cross. We propose a combinatorial and geometric study of multitriangulations based on their stars, which play the same role as triangles of triangulations. This study leads to interpret multitriangulations by duality as pseudoline arrangements with contact points covering a given support. We exploit finally these results to discuss some open problems on multitriangulations, in particular the question of the polytopal realization of their flip graphs. We study secondly the polytopality of Cartesian products. We investigate the existence of polytopal realizations of cartesian products of graphs, and we study the minimal dimension that can have a polytope whose k-skeleton is that of a product of simplices.

==> miscellaneous/titre2NB.tex <==

\cleardoublepage

\thispagestyle{empty}

\vspace*{-8.6cm}\hspace*{12.5cm}\includegraphics[scale=1]{frontpage72}
\vspace*{-25cm}

%\vspace*{-8.5cm}\hspace*{12.5cm}\includegraphics[scale=1]{frontpage82}
%\vspace*{-25cm}

\begin{center}

\vspace*{.3cm}

{\fontseries{m}\fontshape{n}\fontsize{23}{23}\selectfont
%\darkblue
Multitriangulations, pseudotriangulations \\ et quelques problèmes de réalisation de polytopes

\vspace{1.7cm}
%\vspace{1.6cm}

Multitriangulaciones, pseudotriangulaciones \\ y algunos problemas de realización de politopos

\vspace{1.7cm}
%\vspace{1.6cm}

Multitriangulations, pseudotriangulations \\ and some problems of realization of polytopes

}

\vspace{1.5cm}
{\black\rule{7cm}{.5pt}}
\vspace{1.5cm}

{\fontseries{m}\fontshape{sc}\fontsize{22}{22}\selectfont
Vincent Pilaud

}

\vspace{1.8cm}

\begin{minipage}[c]{4.3cm}
\begin{flushright}
sous la direction de \\ bajo la dirección de \\ under the supervision of

\end{flushright}
\end{minipage}
\quad
\begin{minipage}[c]{10.8cm}
\fontseries{m}\fontshape{n}\fontsize{17}{13}\selectfont
\textsc{Michel Pocchiola} \\ {\normalsize École Normale Supérieure, Paris}  \\ {\normalsize Université Pierre et Marie Curie, Paris} \\ \\
\textsc{Francisco Santos Leal} \\ {\normalsize Universidad de Cantabria, Santander}
\end{minipage}

\end{center}
